Transformed Multi-view 3D Shape Features with Contrastive Learning

This paper addresses the challenges in representation learning of 3D shape features by investigating state-of-the-art backbones paired with both contrastive supervised and self-supervised learning objectives. Computer vision methods struggle with recognizing 3D objects from 2D images, often requiring extensive labeled data and relying on Convolutional Neural Networks (CNNs) that may overlook crucial shape relationships. Our work demonstrates that Vision Transformers (ViTs) based architectures, when paired with modern contrastive objectives, achieve promising results in multi-view 3D analysis on our downstream tasks, unifying contrastive and 3D shape understanding pipelines. For example, supervised contrastive losses reached about 90.6% accuracy on ModelNet10. The use of ViTs and contrastive learning, leveraging ViTs' ability to understand overall shapes and contrastive learning's effectiveness, overcomes the need for extensive labeled data and the limitations of CNNs in capturing crucial shape relationships. The success stems from capturing global shape semantics via ViTs and refining local discriminative features through contrastive optimization. Importantly, our approach is empirical, as it is grounded on extensive experimental evaluation to validate the effectiveness of combining ViTs with contrastive objectives for 3D representation learning.

==> tables/image_retrieval_eval.tex <==
\begin{table}[htb]
\centering
\renewcommand*{\arraystretch}{1.2}
\setlength{\tabcolsep}{1.0pt}
\caption{Image retrieval evaluation. We report mAP on the revisited Oxford ($\mathcal{R}$Ox) and Paris ($\mathcal{R}$Par) for the (M) Medium and (H) Hard subsets. For reference, we also report results on ImageNet-pretrained backbones. Top performing in \textbf{bold}.}
\label{tab:image-retrieval}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllccccc}
\toprule
\multicolumn{4}{c}{} & 
\multicolumn{2}{c}{$\mathcal{R}$Ox} & \multicolumn{2}{c}{$\mathcal{R}$Par} \\
\cmidrule(lr){5-6} \cmidrule(lr){7-8}
Method & Backbone & Fine-tuned & Epochs & M & H & M & H \\
\midrule

DINO~\cite{caron2021emerging} & ViT-S/16     & ImageNet   & 800 & \textbf{41.8} & \textbf{13.7} & \textbf{63.1} & \textbf{34.4} \\
DINO~\cite{caron2021emerging} & ResNet-50    & ImageNet   & 800 & 35.4 & 11.1 & 55.9 & 27.5 \\

\midrule

\rowcolor{orange!10} SINCERE (Ours)               & ViT-B/16     & ModelNet10 & 100 & 28.7 & 9.0  & 58.8 & 30.6  \\
\rowcolor{orange!10} $\epsilon$-SupInfoNCE (Ours) & DINO-S/16    & ModelNet40 & 100 & 15.7 & 2.6  & 26.0 & 8.1   \\
\rowcolor{orange!10} SimCLR (Ours)                & DINO-B/16    & ModelNet10 & 100 & 35.6 & 13.4 & 60.4 & 31.9   \\
\rowcolor{orange!10} SimCLR (Ours)                & DINO-B/16    & ModelNet40 & 100 & 35.6 & 13.4 & 60.4 & 31.9   \\

\bottomrule
\end{tabular}
}
\end{table}

==> tables/linear_eval_accs.tex <==
\begin{table*}[htb]
\centering
% \normalsize
\renewcommand*{\arraystretch}{1.2}
\setlength{\tabcolsep}{5.0pt}
\caption{Linear evaluation on Test Set. Performance evaluation Top-1 and Top-5 accuracy (\%) on the test set for ModelNet10 and ModelNet40 datasets using various backbones and contrastive loss functions with supervised and self-supervised settings. Top performing in \textbf{bold} for supervised contrastive losses and top performing for self-supervised contrastive losses in \underline{underlined} relative to each backbone, respectively. We compare our performance with the baseline cross-entropy loss.}
\label{tab:lineareval-acc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\toprule
\multirow{3}{*}{Losses} & \multicolumn{10}{c}{ModelNet10} & \multicolumn{10}{c}{ModelNet40} \\ \cmidrule(lr){2-11} \cmidrule(lr){12-21}
 & \multicolumn{2}{c}{ResNet-50} & \multicolumn{2}{c}{ViT-S/16} & \multicolumn{2}{c}{ViT-B/16} & \multicolumn{2}{c}{DINO-S/16} & \multicolumn{2}{c}{DINO-B/16} 
 & \multicolumn{2}{c}{ResNet-50} & \multicolumn{2}{c}{ViT-S/16} & \multicolumn{2}{c}{ViT-B/16} & \multicolumn{2}{c}{DINO-S/16} & \multicolumn{2}{c}{DINO-B/16} \\
 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 
 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 \\
\midrule
SupCon \cite{khosla2020supcon}                   
& \textbf{80.08} & \textbf{98.02} & 83.24 & 98.84 & 90.49 & 99.67 & 90.16 & 99.48 & 90.14 & 99.59 

& 57.04 & \textbf{77.53} & 80.39 & 96.21 & 84.28 & 95.94 & 85.57 & 97.03 & 83.83 & 96.85 \\

$\epsilon$-SupInfoNCE \cite{barbano2023unbiased} 
& 77.10 & 96.32 & 89.71 & 99.78 & 90.51 & 99.65 & \textbf{90.20} & 99.57 & 90.42 & 99.71 

& \textbf{57.33} & 73.36 & 82.24 & \textbf{97.05} & \textbf{85.89} & \textbf{97.76} & \textbf{86.18} & 97.74 & \textbf{85.68} & \textbf{97.94} \\

SINCERE \cite{Feeney2023sincere}                 
& 78.72 & 96.67 & \textbf{89.91} & \textbf{99.84} & \textbf{90.62} & \textbf{99.73} & 90.18 & \textbf{99.62} & \textbf{90.58} & \textbf{99.82} 

& 56.78 & 74.35 & \textbf{82.27} & 96.99 & 85.60 & 97.42 & 85.93 & \textbf{97.80} & 85.63 & 97.72 \\

\midrule

SimCLR \cite{Chen2020simclr}                     
& \underline{43.62} & \underline{85.18} & \underline{71.40} & 97.49 & 70.64 & 97.65 & \underline{76.49} & \underline{98.41} & \underline{78.82} & \underline{98.67} 

& \underline{32.99} & \underline{64.09} & 66.04 & 90.72 & 69.25 & 92.53 & 71.84 & 93.32 & \underline{75.37} & 94.56 \\

InfoNCE \cite{oord2018infonce}                   
& 41.99 & 83.58 & 70.93 & \underline{97.59} & \underline{71.25} & \underline{97.67} & 75.38 & 98.25 & 78.39 & 98.56 

& 29.77 & 60.54 & \underline{66.43} & \underline{91.17} & \underline{69.60} & \underline{92.57} & \underline{71.98} & \underline{93.57} & 75.19 & \underline{94.58} \\

\midrule
\rowcolor{gray!10}
Cross-Entropy (baseline)
%ModelNet10
& 37.57 & 82.34 & 44.61 & 85.66 & 58.66 & 94.15 & 81.87 & 98.28 & 54.59 & 92.06 
%ModelNet40
& 32.57 & 68.99 & 33.60 & 68.49 & 55.45 & 84.72 & 78.85 & 93.76 & 55.64 & 85.83 \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> tables/map_eval.tex <==
\begin{table}[htb]
\centering
\renewcommand*{\arraystretch}{1.2}
% \setlength{\tabcolsep}{4.0pt}
\caption{3D shape retrieval. We report the mean Average Precision (mAP) and mAP@10. Top performing results in \textbf{bold}. Our approach ViT-B/16 with SINCERE, achieves the best performance among recent SOTA methods using contrastive 3D pipelines on the ModelNet10 dataset with only 12 views. \textcolor{red}{[marcus]: tirar essa tabela!}}
\label{tab:map-metrics}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Method & \# of Views & mAP & mAP@10 \\
\midrule

\textcolor{gray}{\textit{ModelNet10}} & & & \\

\acrshort{cmvlnet} \cite{peng2024contrastive} & 12 & -- & -- \\
\rowcolor{orange!10} \textbf{ViT-B/16 with SINCERE (Ours)} & 12 & \textbf{95.5} & \textbf{96.6} \\
\rowcolor{orange!10} \textbf{DINO-B/16 with SimCLR (Ours)} & 12 & 51.4 & 90.8 \\

\midrule

\textcolor{gray}{\textit{ModelNet40}} & & & \\

MVCNN \cite{su2015multi} & 12 & 70.1 & -- \\
MVTN \cite{hamdi2021mvtn} & 12 & \textbf{92.9} & -- \\
EMVN \cite{esteves2019equivariant} & 12 & 91.8 & -- \\
MVCL \cite{li2025multi} & 12 & -- & -- \\
\acrshort{cmvlnet} \cite{peng2024contrastive} & 12 & -- & -- \\
\rowcolor{orange!10} \textbf{DINO-S/16 with $\epsilon$-SupInfoNCE (Ours)} & 12 & 58.7 & 87.3 \\
\rowcolor{orange!10} \textbf{DINO-B/16 with SimCLR (Ours)} & 12 & 50.7 & \textbf{89.3} \\

\bottomrule
\end{tabular}
\smallskip
\begin{minipage}{\linewidth}
% \footnotesize ``-" represents missing metric.
\end{minipage}
}
\end{table}

